A Methodology for Evaluating RAG Systems: A Case Study On Configuration Dependency Validation

Retrieval-augmented generation (RAG) is an umbrella of different components, design decisions, and domain-specific adaptations to enhance the capabilities of large language models and counter their limitations regarding hallucination and outdated and missing knowledge. Since it is unclear which design decisions lead to a satisfactory performance, developing RAG systems is often experimental and needs to follow a systematic and sound methodology to gain sound and reliable results. However, there is currently no generally accepted methodology for RAG evaluation despite a growing interest in this technology. In this paper, we propose a first blueprint of a methodology for a sound and reliable evaluation of RAG systems and demonstrate its applicability on a real-world software engineering research task: the validation of configuration dependencies across software technologies. In summary, we make two novel contributions: (i) A novel, reusable methodological design for evaluating RAG systems, including a demonstration that represents a guideline, and (ii) a RAG system, which has been developed following this methodology, that achieves the highest accuracy in the field of dependency validation. For the blueprint's demonstration, the key insights are the crucial role of choosing appropriate baselines and metrics, the necessity for systematic RAG refinements derived from qualitative failure analysis, as well as the reporting practices of key design decision to foster replication and evaluation.

==> old/1-introduction.tex <==
\section{Introduction}
%%% Configuration Dependencies
Modern software development involves a plethora of technologies that developers must coordinate to create, build, test, and deploy software systems. These technologies include code frameworks, containerization technologies, build tools, databases, and continuous integration and delivery pipelines~\cite{sayagh2017cross}. The coordination is usually conduct around configuration of each technology in its own format. For instance, container configuration is defined in \texttt{Dockerfile} and Java application options are set in \texttt{applications.yml}. These configuration files often encode hundreds of configuration options in their own structure, syntax, and semantic~\cite{siegmund2020dimensions}, which alone can be complicated and error-prone~\cite{xu2015hey}. Even more challenging, most of these diverse technologies' configurations need to be harmonized to ensure their correct interplay and interoperability, such as the port configuration in the \texttt{application.yml} in Listing~\ref{lst:example-application} and the \texttt{Dockerfile} in Listing \ref{lst:example-docker}. In this exemplary Spring Boot application scenario, the port resembles a \textit{configuration dependencies}, because both options must align to work properly. In practice, configuration dependencies not only exist across (cross-) technologies, but also within a single (intra-) technology.

\begin{figure}[ht]
\centering
 \begin{minipage}[t]{0.48\columnwidth}
  \centering
  \begin{lstlisting}[language=Spring, label=lst:example-application, caption=Spring Boot's application.yml specifying the port of the web server.]
server:
  port: 8080
spring:
  application:
    name: app
\end{lstlisting}
 \end{minipage} \hfill % Fill horizontal space between the minipages
 \begin{minipage}[t]{0.48\columnwidth}
   \centering
    \begin{lstlisting}[language=Dockerfile, label=lst:example-docker, caption=A Dockerfile exposing the port of the web server.]
FROM openjdk:11-jdk-slim
ARG JAR_FILE=target/*.jar
ADD ${JAR_FILE} app.jar
EXPOSE 8080
CMD ["java", "-jar", "/app.jar"]
\end{lstlisting}
 \end{minipage}
\caption{An exemplary cross-technology configuration dependency between Spring-Boot and Docker, both specifying the port of the web server.}
\end{figure}

%%% Configuration Errors
Naturally, developers of these technologies cannot meticulously manage all the frameworks and tools that potentially interact in their technology stack. Consequently, configuration dependencies are rarely fully documented~\cite{chen2020understanding} and the corresponding documentations are commonly found to be incomplete and outdated~\cite{hubaux2012user, jin2014configurations, rabkin2011static}. As a result, there is no comprehensive overview about how and where configuration dependencies manifest within a software project. The absence of a comprehensive overview of the intertwined configuration dependencies poses several challenges in practice:
(1)~the rapid evolution of software technologies leads to an ever-evolving configuration landscape and frequent configuration changes, bearing the risk of introducing severe misconfigurations~\cite{maurer2015fail, tang2015holistic, mehta2020rex};
(2)~misconfigurations may go unnoticed due to the interplay of multiple technologies that manifest themselves only in combination  (e.g., often only in production);
(3)~the resulting configuration errors are complex and far-reaching since several technologies and diverse configuration artifacts are involved~\cite{yin2011empirical, xu2015systems};
(4)~the detection and resolution of such misconfigurations is often more challenging than fixing software bugs, making misconfigurations one of the most common causes of software failures in production today~\cite{oppenheimer2003internet, gunawi2016does, rabkin2012hadoop}. For example, a minor configuration change at Facebook in 2021 led to a serious misconfiguration incident that caused all Facebook services to be unavailable for about six hours~\cite{facebook_misconfiguration}. 

%%% Existing approaches
 %For example, \emph{CfgNet}~\cite{simon2023cfgnet} leverages an equality-based heuristic to detect intra- and cross-technology dependencies in a software projects. That is, it flags configuration options with the same value as dependencies. However, this heuristic bears the risk of creating many false positives, as configuration options may have equal values by chance without an actual dependency. \emph{CfgNet} incorporates several mechanisms to mitigate the risk of false positives, but these mechanisms are developed with significant technical effort and are not technology- and dependency-agnostic.

% Our goal
In this work, we set out to boost practicality, applicability, and generalizability that existing dependency-detection approach lack by automating the validation of configuration dependencies in a technology-independent way. We achieve this by backing the comprehension capabilities of large language models (LLMs) with relevant contextual information through retrieval-augmented generation (RAG) to accurately identify true configuration. Trained on massive amounts of data, such as software repositories, blog posts, and Q\&A websites, LLMs already encode common configuration knowledge, making them a promising tool for handling the configuration of modern software stacks. 

% Related work
The potential of LLMs for configuration validation has already been tapped by \citeauthor{lian2023configuration}~\cite{lian2023configuration}, which validate single configuration files to detect constraint and dependency violations. While LLMs showed promising results in validating constraint violations, they exhibit difficulties in validating dependency violations du to missing contextual information. We therefore state the following question: \emph{Does providing additional contextual information improve the effectiveness of LLMs in validating configuration dependencies?}

% Experiments
To address this question, we developed an extensive RAG system for dependency detection in configuration files. In a large scale empirical study, we assess whether our approach can reduce false positives of ex existing dependency detection framework. Specifically, we validate 500 configuration dependencies extracted with \emph{CfgNet}~\cite{simon2023cfgnet} from ten real-world software projects that incorporate a microservice technology stack based on Spring Boot. To further evaluate the role of RAG and LLM size, we used four state-of-the-art LLMs combined with different RAG variants, incorporating contextual information from technology manuals, Stack Overflow posts, GitHub repositories, and Web searches. This provides crucial empirical insights whether providing additional contextual information enhances the effectiveness of LLMs in validating configuration dependencies. Furthermore, we qualitatively analyze the validation results to identify common patterns where LLMs still fail to validate dependencies, with and without additional contextual information. Based on our findings, we derive recommendations on the specific contextual information needed for accurate validation of configuration dependencies by LLMs.

%%% Results
Our evaluation results show a mixed picture: ...

%%% Contribution
In summary, we make the following contributions:

\begin{compactitem}
    \item We developed a RAG system to explore the effectiveness of LLMs complemented with RAG in validating configuration dependencies, showing the effect of additional contextual information on the dependency validation effectiveness of LLMs.
    \item We conduct an extensive qualitative analysis on the validation results of LLMs, identifying common patterns where LLMs are effective or fail to validate dependencies.
    \item We derive recommendations about which contextual information is actually required to validate configuration dependencies using LLMs and prove them.
    \item We provide a replication package containing all code, data sets, prompt templates, and evaluation results on TBA.
\end{compactitem}

Note that our findings go beyond the application of dependency detection as the effectiveness of the relatively novel approach of RAG systems for software engineering tasks is not yet extensively researched. We provide with our study an important piece to the puzzle by analyzing which context information of different RAG settings influence the outcome of the software engineering task.




==> old/3-related-work.tex <==
\section{Related Work}
In this section, we discuss related work on dependency extraction, configuration validation, and LLMs for tackling software configuration.

\paragraph{\textbf{Configuration Dependency Detection}}
The challenge of detecting and extracting configuration dependencies in software systems has inspired several research approaches.
A common method relies on machine learning. For example, ConfigC~\cite{santolucito2016probabilistic} and ConfigV~\cite{santolucito2017synthesizing} use an advanced form of association rule learning to learn different kinds of configuration rules. These approaches identify both coarse- and fine-grained value dependencies between configuration options in MySQL configuration files.

\citeauthor{chen2020understanding}~\cite{chen2020understanding} conducted a comprehensive study on configuration dependencies in 16 widely-used software projects across two different cloud- and data-center software stacks. They analyzed configuration metadata and manual pages of these projects, identifying intra- and cross-component configuration dependencies, common code patterns, potential impacts, and existing dependency-checking practices. Based on these findings, they developed cDep, a framework that identifies configuration dependencies within and across software components using static taint analysis. \citeauthor{simon2023cfgnet}~\cite{simon2023cfgnet} conducted a systematic literature study to explore the various forms of configuration constraints and dependencies within software projects. Their literature study highlights value-equality as a significant and common form of cross-technology dependency in academic literature. To early detect and track equality-based configuration dependencies, they propose CfgNet, a framework that models a software project and its surrounding ecosystem (i.e., technologies such as CI/CD pipelines, build tools, and code frameworks) as a configuration network. By checking the changes in a configuration network, CfgNet enables the early detection of potential dependency violations. \citeauthor{ramachandran2009determining}~\cite{ramachandran2009determining} provide deeper insights into conf\-iguration-parameter dependencies between different component instances of software projects. By analyzing configuration data accessed via APIs, they estimate potential candidates of configuration dependencies, compute weights for each dependency using a heuristic, and provide a ranked list of dependencies. This ranking helps administrators quickly identify and address the most critical dependencies. The framework Rex~\cite{mehta2020rex} combines machine learning and program analysis to identify correlations between code and configuration files across different components in large services. Specifically, Rex employs association rule learning on historical information to determine frequently changed files and then leverages differential syntax analysis to learn change rules, which capture sets of correlated changes across these files. Rex then analyzes these change rules to suggest additional required changes.

While all the aforementioned approaches contribute valuable solutions for detecting configuration dependencies in software systems, they often produce many false positives, reducing accuracy and applicability of these approaches. To mitigate the risk of false positives, these approaches usually incorporate additional validation techniques. However, these validation mechanisms demand extensive technical effort and are limited to single projects, a small set of technologies, and specific kinds of dependencies. By contrast, our goal is to enable automated dependency validation that generalizes to various software systems, technology environments, and forms of configuration dependencies using LLMs in combination with RAG, without requiring manual engineering, which increases the applicability of the aforementioned approaches.

\noindent \paragraph{\textbf{Configuration Validation}}
As misconfigurations are a leading cause of software failures in production, several research approaches aim to validate configurations to proactively detect misconfigurations. A common method relies an domain-specific languages to describe configuration specification rules. For example, ConfValley by \citeauthor{huang2015confvalley}~\cite{huang2015confvalley} is a configuration validation framework that includes a declarative language for describing configuration specifications, an inference engine for automatically generating these specifications, and a checker engine for determining if a given configuration matches its specification. In a similar way, \citeauthor{baset2017usable}~\cite{baset2017usable} propose ConfigValidator, which uses a declarative language to write rules for detecting various misconfigurations. Both approaches require manual engineering to define specification rules. By contrast, we focus on an automated validation of configuration dependencies using LLMs, eliminating the need for manual rule engineering.

The work most closely related to ours is that of Lian et. al~\cite{lian2023configuration}, which investigates the feasibility and effectiveness of using LLMs for configuration validation. They introduce Ciri, a generic LLM-based framework, to validate configurations to detect constraint and dependency violations in single configuration files. Based on effective prompt engineering with few-shot learning including both correct and incorrect configuration data, Ciri detects and validates constraint and dependency violations within a single configuration file at both the file and parameter level. Their experiments on six open-source software systems showed promising results. However, they identified limitations in recognizing certain misconfigurations, such as dependency violations, due to their inherent nature. While constraint violations (e.g., syntax and value range) are more common, dependency violations are often technology-specific and harder for LLMs to capture without fine-tuning on dependency-related data. Unlike the approach by Lian et al.~\cite{lian2023configuration}, our approach can be combined with existing dependency-detection techniques to automate the validation of detected configuration dependencies. Our approach leverages LLMs combined with a RAG system solely for validation, eliminating the need for LLMs to detect configuration dependencies before validation. Another key difference is that \citeauthor{lian2023configuration}~\cite{lian2023configuration} focus mainly on constraint and dependency violations within single configuration files, while our approach focuses on validating configuration dependencies across multiple technologies.


\noindent \paragraph{\textbf{LLMs for Tackling Software Configuration}}
LLMs are promising tools for handling software configuration. For instance, DB-Bert by Trummer~\cite{trummer2022db} employs a pre-trained LLM (i.e., a BERT model) to extract domain knowledge gained from relevant text sources, such as manuals, to identify database systems parameters for tuning and recommended parameters values. \citeauthor{lao2023gptuner}~\cite{lao2023gptuner} introduce GPTuner, a database tuning system that enhances the optimization process of database management systems (DBMS) by leveraging domain knowledge obtained through an LLM-based pipeline and a prompt ensemble algorithm. Similarly, LLMTune~\cite{huang2024llmtune} recommends high-quality initial configurations tailored to a new database tuning task based on previous tuning tasks of DB administrators. \citeauthor{liu2024llm}~\cite{liu2024llm} propose LLM-CompDroid, which uses LLMs alongside traditional bug resolution tools to detect and repair configuration compatibility bugs in Android apps. \citeauthor{shan2024face}~\cite{shan2024face} introduce LogConfigLocalizer, which leverages LLMs to localize root-cause configuration dependencies through log analysis. Additionally, \citeauthor{wang2024identifying}~\cite{wang2024identifying} developed PerfSense, which leverages LLMs to identify performance-sensitive configurations. By utilizing LLM agents and advanced prompting techniques, such as prompt chaining and retrieval-augmented generation, PerfSense mimics the interaction between developers and performance engineers to classify configurations based on their performance sensitivity.

All of the aforementioned approaches demonstrate the potential of LLMs in tackling various tasks related to software configuration. Similarly, our work explores the capabilities of LLMs combined with an external knowledge base, but we focus specifically on validating intra- and cross-technology configuration dependencies, setting our approach apart from other presented efforts.

==> old/4-experiment.tex <==
\section{Experiment Setup}
Our goal is to assess whether providing additional contextual information to LLMs enhance their effectiveness in validating configuration dependencies. To this end, we conduct a series of experiments using an existing dependency-detection framework to extract configuration dependencies from ten real-world software projects and validate a sample set of dependencies 
with our approach. In what follows, we describe our research questions, the dependency datasets, and the operationalization of our experiments.

\subsection{Research Questions}

\begin{tcolorbox}[myboxstyle, title=RQ 1: Dependency Validation Effectiveness of RAG]
Does providing additional contextual information to LLMs improve their effectiveness in validating intra- and cross-technology configuration dependencies?
\end{tcolorbox}

Inspired by related work on configuration validation~\cite{lian2023configuration} and the importance to detect true dependencies, we aim to explore whether providing additional contextual relevant information reduces false positives. Note since we provide an extension to existing dependency-detection frameworks, we cannot review false negatives as these non-dependencies are not provided by dependency-detection frameworks. For a sound empirical analysis, we compare compare the effectiveness of various LLMs with and without additional contextual information obtained through different RAG variants in validating configuration dependencies. Specifically, we experiment with four different state-of-the-art LLMs (i.e., GPT-4o, GPT-3.5-Turbo, Llama3:8b, and Llama3:70b) and four different variants of RAG. The RAG variants differ in critical components, such as embedding model, re-ranking algorithm, and the final number of retrieved context information used for augmentation. This allows us to study the effect of additional contextual information across different model architectures and sizes, yielding generalizable results. Thus, our first research question aims at assessing whether providing additional contextual information to LLM enhances their effectiveness in validating configuration dependencies.

\begin{tcolorbox}[myboxstyle, title=RQ 2: In-depth Failure Analysis]
What validation failures occur in LLMs with and without additional contextual information, and what specific contextual information is necessary to enhance the effectiveness of configuration dependency validation by LLMs?
\end{tcolorbox}

Besides quantitative results on the validation effectiveness of LLMs, we further investigate the validation results of LLMs qualitatively. With RQ2, we therefore take a closer look at the LLM responses of the LLM and RAG variant that achieved the highest validation scores. Specifically, we qualitatively analyze the corresponding LLM responses generated with and without additional contextual information to determine when the LLM performs particularly well and when it fails. Based on our findings, we derive recommendations on the specific contextual information needed for accurate validation of configuration dependencies by LLMs.

\subsection{Dependency Datasets}
To answer our research questions, we need a dataset containing configuration dependencies and ground truth labels that can be validated with our approach. We therefore searched for software projects with technologies that have potential configuration dependencies across the entire technology stack and are covered by a previously published dependency-detection tool. We decided to to use \emph{CfgNet}~\cite{simon2023cfgnet} as a tool, as it is technology-agnostic and supports many state-of-the-art technologies. For the technology stack, we selected software projects that incorporate a microservice technology stack within the Spring Boot ecosystem.

\paragraph{\textbf{Subject Systems}}
The selection of software projects was driven by the usage of the ecosystem and the activity as well as star count in GitHub. This way, we obtain highly practical, real-world use cases for our evaluation. Using GitHub Topics~\footnote{\url{https://github.com/topics}}, we obtain over 60,000 public repositories in the Spring Boot ecosystem. We sorted these projects by stars and included those incorporating at least the following technologies: Spring Boot, Maven, Docker, and Docker Compose. We stopped the selection after identifying 10 suitable projects with these technologies. The resulting subject systems and their characteristics are shown in Table~\ref{tab:subject-systems}.

\input{tables/table-subject-systems}

\paragraph{\textbf{Extracting Dependencies from Subject Systems}}
To get a dataset of configuration dependencies from our subject systems, we apply CfgNet to all of them and extract all potential configuration dependencies. For each software project, we randomly select 50 configuration dependencies from the detected ones, resulting in a set of 500 intra- and cross-technology dependencies for our evaluation. The rational for this sampling is that all dependencies must be manually checked in detail to create a trustworthy and correct ground truth. \added{That is, the main author manually reviewed all dependencies and annotated them as either\emph{true}, a \emph{false}, or as \emph{borderline} case. \emph{Borderline} cases were discussed by at least two authors until a consensus in favor of a \emph{true} or \emph{false} dependency was found. This way, we created the largest ground truth cross-technology configuration dependency dataset that we are aware of and that have been used in any evaluation. As an important contribution of this work, we make this dataset available for other researchers and tool developers.}

\subsection{Operationalization}
To answer our research question, we conduct two experiments, one per research question, using a dependency dataset created with \emph{CfgNet}. Throughout the first experiment, we vary between four state-of-the-art LLMs to assess the validation effectiveness with and without additional contextual information of different LLMs. Two of the LLMs are proprietary and developed by OpenAI\footnote{\url{https://openai.com/}}: (1) GPT-4o; (2) GPT-3.5-Turbo. The other two LLMs are open-source and developed by Meta\footnote{\url{https://llama.meta.com/llama3/}}: (3) LLama3:8b; (4) LLama3:70b (non-quantized), executed on our own hardware, a MacBook Pro with an Apple M3 chip. A summary of the studied LLMs with their properties can be found in Table~\ref{tab:models}. For all LLMs, we set the temperature to 0 in order to improve determinism and consistency of LLM outputs. We make all experiment scripts, dependency datasets, prompt templates, and validation results available on the paper’s supplementary website TODO.

\input{tables/table-models}


% revise
\paragraph{\textbf{Experiment 1 (RQ1)}}
We prompt all four LLMs to validate our sample set of dependencies with and without RAG. We thereby experiment with four RAG variants that differ in the embedding model, re-ranking algorithm, and number of context chunks provided to the LLM. Note that we are not conceptually limited to these components, but consider them as crucial components of a RAG system. Table~\ref{tab:rag-configs} summarizes all RAG variants employed in our first experiment. Overall, we conduct 20 experiments runs, in each of which we validate 500 configuration dependencies. For each experiment run, we automatically compute the precision, recall, and F1-score by counting true positives (TP), false positives (FP), true negatives (TN) and false negatives (FN) against the ground truth. We provide a definition of the confusion matrix terms in Table ~\ref{tab:metrics-definitions}. 


\input{tables/table-rag-configs}

\input{tables/table-metrics-definitions}

\paragraph{\textbf{Experiment 2 (RQ2)}}
We answer RQ2 by manually analyzing LLM responses created in the first experiment with the LLM and RAG variant that achieved the highest validation effectiveness. We manually review LLM responses and derive failure categories to identify where the LLM performs particularly well and where it fails, highlighting the current limitations and strengths of LLMs in validating configuration dependencies. Based on our findings we derive recommendations on the specific contextual information needed for accurate validation of configuration dependencies by LLMs. We prove our recommendations by testing them on the falsely validated dependencies.


%\paragraph{\textbf{Experiment 2 (RQ2)}}
%In RQ2, we explore whether and how context sources on which developers typically rely when facing dependency-related issues contain contextual information about configuration dependencies. We experiment with static and dynamic context information. As static context information, we include technology manuals, Stack Overflow posts, and configuration data from the corresponding GitHub repositories that we selected as subject systems. All this context information was collected and indexed into vector database in advance to the experiments. Conversely, dynamic context information is scraped from the web and index for each dependency during validation. As LLM and retrieval-augmented generation variant, we us the combination that achieved the highest validation effectiveness in our first experiment. This results in X experiments, one per data source (i.e., technology manual, Stack Overflow posts, GitHub repositories, and web search). For each experiment run, we again compute the accuracy, precision, recall, and F1-score by counting true positives, false positives, true negatives and false negatives against the manually annotated labels. Additionally, we assess the generated validation responses of LLM using the answer and context relevancy metrics from DeepEval~\footnote{\url{https://docs.confident-ai.com/}} to measure the relevance of the LLM's responses and the retrieved context on the provided input to the LLM. 

==> old/4-method.tex <==
\section{Dependency Validation via Retrieval-Augmented Generation} %RAG Architecture -> evtl ins Kapitel mit Szenario
In this section, we present the architecture of the RAG system to validate configuration dependencies. Figure~\ref{fig:method} illustrated the process of indexing static and dynamic contextual information into a vector database, through retrieving relevant contextual information from it, to querying an LLM with an augmented prompt containing the given dependency and additional contextual information. 

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/method_cropped.pdf}
    \caption{An overview of indexing contextual information into a vector database, retrieving additional contextual information from it, and querying an LLM with an augmented prompt to validate a configuration dependency.}
    \label{fig:method}
\end{figure}

\subsection{Context Ingestion}
Our goal is to investigate whether augmented prompts with contextual information improves the validation effectiveness of LLMs. So, acquisition and ingestion of information about configuration dependencies into a vector database is a paramount component. The main challenge for this is that relevant information about configuration dependencies is rarely available and usually not explicitly stated. For example, manuals typically describe configuration options in terms of their names, abbreviations, functionally, and (rarely) their allowed parameter ranges. But the description almost always lacks explicit dependency information to other options of that technology and entirely to other technologies. So, developers turn to Stack Overflow that contain practical usages in which concrete dependencies are explicitly or implicitly discussed. Based on such scarcely distributed knowledge, we collect information from various sources and store it into a vector database, including technology manuals, Stack Overflow posts, GitHub repositories, and a Web search results.

We differentiate between static and dynamic context information. \emph{Static} context information is pre-stored in the vector database before validating configuration dependencies. It includes data from technology manuals, Stack Overflow, and GitHub repositories. \emph{Dynamic} context information is scraped from the Web, processed, and indexed into the vector database on-the-fly for each dependency during validation. 

\paragraph{\textbf{Static Context}}
Before validating dependencies, we populate a vector database with static context information from technology manuals, Stack Overflow posts, and corresponding GitHub repositories. These context sources have to be mined in advance based on the subject systems to analyze and the technologies they incorporate. The resulting context information from these sources is transformed into documents, a generic container that stores text along with metadata, using a data loader from llama-index\footnote{\url{https://www.llamaindex.ai/}}.

The resulting documents are then split into smaller chunks with a certain amount of overlap. We choose a chunk size of 512 with an overlap of 50 in order to encompass all necessary information in the retrieved chunks. After splitting, the resulting chunks are then converted into embeddings, a vector representation of the documents, using an embedding model. Finally, the resulting embeddings are indexed into a vector database. 

\paragraph{\textbf{Dynamic Context}}
We also dynamically obtain context information from the Web for each validation task. When validating a given dependency, we query the web with the characteristics of the dependency, including the involved technologies, option names, and currently set values, to retrieve websites with possibly relevant information. Specifically, we employ DuckDuckGo\footnote{\url{https://duckduckgo.com/}} as search engine and a web reader from llama-index. For each query, we convert the first three search results them into documents. The documents are then split into smaller chunks and converted into embeddings to index them into the vector database. 

\subsection{Dependency Validation}
Starting with a detected dependency by a dependency-detection framework, we first retrieve relevant contextual information from the vector database using the characteristics of the dependency. This includes information from the static context as well as from the dynamic web search for the given dependency. We then inject the dependency and retrieved contextual information into a prompt template and query the LLM with the augmented prompt to validate the given dependency. Finally, we receive a LLM response indicating a true dependency or a false positive, along with a plan describing the validation procedure, a rationale explaining whether the configuration options depend on each other, and a rating of uncertainty about the configuration dependency.

\paragraph{\textbf{Context Retrieval}}
To retrieve relevant context for a given dependency, we introduce several retrieval strategies to enhance retrieval quality. First, we optimize the original query by rewriting. We then perform a hybrid search in the vector database with the retrieval query to obtain an initial set of contextual information. With a hybrid search, we combine a semantic and a keyword search in one query, allowing us to capture different relevance features, such as keyword and semantic equality, with our retrieval query. After obtaining an large initial set of contextual information, we re-rank the elements of this set such that the most relevant information comes first. Finally, we use the re-ranked contextual information to augment the prompt for dependency validation.

\paragraph{\textbf{Prompt Generation}}
We created a prompt for dependency validation using a collective prompt design process, in which all authors discussed and adjusted the prompt and its components in multiple iterations. Our final prompt for dependency validation includes five elements: (1) a system message that defines the role of the LLM and (2) a definition of the dependency that it receives for validation, (3) contextual information that is retrieved from a vector database for a given dependency using a hybrid search, (4) the actual validation instruction for a given dependency, and (5) a description of the JSON format in which the LLM should respond. The validation prompt and its components is shown in \autoref{fig:prompt}. The bold text between curly brackets is replaced by the corresponding information of a given dependency and the retrieved contextual information.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/prompt_template_cropped.pdf}
    \caption{The prompt template and its components used for dependency validation.}
    \label{fig:prompt}
\end{figure}


\paragraph{\textbf{Validation Generation}}
We instruct an LLM to validate a given dependency by generating a validation response in JSON format that contains four primary fields: (1) \emph{plan}: a string that describes the plan on how to validate the dependency based on the contextual information step-by-step; (2) \emph{rationale}: a string that explains whether and why the configuration options depend on each other or not; (3) \emph{uncertainty}: an integer from 0 (completely uncertain) to 10 (absolutely certain) that indicates the LLM's uncertainty about the dependency based on the context information, \emph{plan}, and \emph{rationale}; and (4) \emph{isDependency}: a boolean indicating the final decision of the LLM whether the given dependency is a true dependency or a false positive. 

% add reference for uncertainty key
The response structure follows the idea of chain-of-thought prompting~\cite{wei2022chain}, aiming to increase the understanding and analytical capabilities of LLMs in validating configuration dependencies. That is, we prompt the LLM to lay out a step-by-step strategy on how to validate the given dependency and to provide an explanation and rating of its uncertainty of before making the final decision. By breaking down the validation task into several steps, each building on the previous one, we ensure a logical progression of actions that the LLM should perform, thereby following prompting best practices TODO. Furthermore, by requiring an explanation and rating of its uncertainty, we encourage a critical and reflective assessment about the dependency and the reliability of the conclusions. Consequently, this response structure naturally encourages a thorough and logical validation of a given dependency following existing prompt engineering techniques.


==> old/5-results.tex <==
\section{Results}
In this section, we present the results of validating configuration dependencies from ten real-world software projects using LLMs complemented with and without RAG. In what follows, we present the results of our experiments to answer our research questions.

\subsection{RQ\textsubscript{1}: Dependency Validation Effectiveness}



\greybox{\textbf{Finding 1:} \textit{Validation effectiveness of LLMs barely varies across different RAG variants}}
- validation effectiveness of models barely varies between different RAG variants
- GPT-4o shows consistent performance across RAG variants, with accuracy and F1-Score remaining stable
- models like llama3:8b show little variations
- noticeable drop of recall in RAG variant 4 for llama3 model compared to other RAG variants
- less context seemingly decreases the recall of llama models, while more context increases recall
- the variability suggests that specific RAG combinations may be better suited for specific models
- therefore tuning RAG components is worth to explore
- big picture does not change (only small differences across RAG variants)
- RAG config 2 performs best (best scores, lowest number of failures)

\greybox{\textbf{Finding 2:} \textit{Lower the precision, higher recall}}
- noticeable pattern between precision and recall across the different RAG variants
- Table~\ref{tab:validation-effectiveness} shows the precision, recall, and F1-score for each RAG variant and without RAG
- precision of all LLMs decreases with RAG, while the recall increases for all LLMs except for GPT-4o
- adding additional contextual information helps LLMs in detecting more true dependencies, but also leads to more false positives.
- pattern can be seen especially across smaller models (gpt-3.5-turbo, llama3:70b, and llama3:8b)


% Einfluss Modellgröße auf Ergebnis mit und ohne RAG
\greybox{\textbf{Finding 3:} \textit{Model size does not always correlate with better performance}}
- gpt-4o outperforms all other models in almost every metric with and especially without RAG
- recall pf gpt-4o is worse compared to other models
- it suggests that larger models are generally more capable of comprehending and processing complex and manifold configuration dependencies
- however, among the other models, larger models do not always outperform smaller models
- llama3:8b outperforms llama3:70b without context, but as far as context is added it is vice versa


\begin{mdframed}[roundcorner=0pt]
\textbf{Answer RQ\textsubscript{1}:} 
- RAG does not always improve effectiveness
- performance of models from the gpt-family slightly decreases
- performance of models from llama-family slightly increases, since the recall increases with additional context
\end{mdframed}


\subsection{RQ\textsubscript{2}:In-depth Failure Analysis}


\greybox{\textbf{Finding 4:} \textit{Inconsistent LLM responses}}
- LLMs produce inconsistent responses for dependencies in the same category
- more inconsistencies with more context? 


\greybox{\textbf{Finding 4:} \textit{The retrieved context is relevant regarding the involved options. However, regardless the context source, the context rarely contains dependency related information, as most dependencies are highly project-specific.}}

%\greybox{\textbf{Finding 2.1:} \textit{Failures without RAG}}

%\greybox{\textbf{Finding 2.2:} \textit{Failures with RAG}}

%\greybox{\textbf{Finding 2.3:} \textit{Context Relevancy}}

%\greybox{\textbf{Finding 2.4:} \textit{Combination with and without RAG}}

%\begin{mdframed}[roundcorner=0pt]
%\textbf{Answer RQ\textsubscript{3}:} \textit{TODO}
%\end{mdframed}


==> old/5-study-design.tex <==
\section{Study Design}
In this section, we describe our research questions, study procedure, and dependency datasets in detail. We make all source code scripts, dependency datasets, prompt templates, and validation failures available on the paper’s supplementary website.

\subsection{Research Questions}

\begin{tcolorbox}[myboxstyle, title=RQ 1: Dependency Validation Effectiveness of Vanilla LLMs]
How effective are vanilla LLMs in validating configuration dependencies?
\end{tcolorbox}

Inspired by related work on configuration validation~\cite{lian2023configuration}, we aim to explore the effectiveness of vanilla LLMs in validating configuration dependencies. For a sound empirical analysis, we compare the effectiveness of various LLMs configuration dependencies. Specifically, we experiment with four different state-of-the-art LLMs (i.e., GPT-4o, GPT-3.5-Turbo, Llama3:8b, and Llama3:70b). This allows us to study the validation effectiveness across different model architectures and sizes, yielding generalizable results.

\begin{tcolorbox}[myboxstyle, title=RQ 2: Dependency Validation Effectiveness of RAG]
Does providing additional contextual information to LLMs improve their effectiveness in validating configuration dependencies?
\end{tcolorbox}

As configuration dependencies are usually highly project- and technology-specific, augmenting LLMs with additional contextual information might be key for enhancing their validation effectiveness of configuration dependencies. To this end, we construct different RAG variants to explore the effect of different RAG components on the validation effectiveness of LLMs. Here, we include static and dynamic contextual information from different sources, such as manuals, Stack Overflow posts, GitHub repositories, and Web search results, to provide the LLM with additional contextual information on the validation tasks. 

\begin{tcolorbox}[myboxstyle, title=RQ 3: Qualitative Validation Failure Analysis]
What validation failures occur with vanilla LLMs and RAG, and what specific contextual information is necessary to enhance the effectiveness of LLMs in validating configuration dependencies?
\end{tcolorbox}

Besides quantitative results on the validation effectiveness of vanilla LLMs and different RAG variants, we further investigate the validation errors of vanilla LLMs and RAG qualitatively. Specifically, we take a closer look at the validation errors of vanilla LLMs and the RAG variant that achieved the highest validation scores. We aim to identify when and why LLMs fail to validate configuration dependency by deriving failure categories. Based on these categories, we derive new contextual information from which a RAG system for dependency validation would benefit.

\subsection{Study Procedure}
We study the benefits of RAG compared to vanilla LLMs on validating configuration dependencies using a three-step approach. We first analyze the ability of vanilla LLMs in validating configuration dependencies. We then construct different RAG variants to explore the effect of different RAG components on the validation effectiveness of LLMs. Finally, we qualitative analyze the validation failures of vanilla LLMs and the best performing RAG variant in terms of validation scores to derive new contextual information from which a RAG system for dependency validation would benefit.

Throughout the first and second step, we leverage four state-of-the-art LLMs, including two proprietary LLMs developed by OpenAI\footnote{\url{https://openai.com/}} (i.e., GPT-4o and GPT-3.5-Turbo) and two open-source LLMs developed by Meta\footnote{\url{https://llama.meta.com/llama3/}} (i.e., LLama3:8b and LLama3:70b (non-quantized)). The open-source LLMs are executed on our own hardware, a MacBook Pro with an Apple M3 chip. A summary of the studied LLMs with their properties can be found in Table~\ref{tab:models}. For all LLMs, we set the temperature to 0 in order to improve determinism and consistency of LLM outputs.

\input{tables/table-models}

\paragraph{\textbf{Step 1: Dependency Validation with Vanilla LLMs}}
In our first step, we investigate the effectiveness of four state-of-the-art LLMs in validating configuration dependencies. To this end, we prompt all four LLMs solely with a task description, including the detected dependency from the dependency-detection tool, and a response format for all dependencies in our dataset. For each LLMs, we compute its validation effectiveness in terms of precision, recall, and F1-score by counting the true counting true positives (TP), false positives (FP), true negatives (TN) and false negatives (FN) against the ground truth labels. We provide a definition of the confusion matrix terms in Table ~\ref{tab:metrics-definitions}. 

\input{tables/table-metrics-definitions}

\paragraph{\textbf{Step 2: Dependency Validation with RAG Systems}}
In our second step, we construct several RAG variants to explore the effect of different RAG components on the validation effectiveness of LLMs. 
Specifically, our RAG variants differ in critical components, such as embedding model, re-ranking algorithm, and the final number of retrieved context information used for augmentation. Table~\ref{tab:rag-configs} shows an overview of the RAG variants that we evaluate on dependency validation.  

\input{tables/table-rag-configs}

\paragraph{\textbf{Step 3: Qualitative Validation Failure Analysis}}
In our third step, we qualitative analyze and compare the validation failures of vanilla LLMs and the best performing RAG system for dependency validation in terms of achieved validation scores. When analyzing the validation errors, we derive failure categories based on the dependencies validated as incorrect. This allows us to identify current limitations of LLMs in validating specific configuration dependencies. From the failure categories, we then derive new contextual information from which a a tailored RAG system would benefit. We integrate the new contextual information in the best found RAG for the validation task and evaluate it.


\subsection{Dependency Datasets}
To validate configuration dependencies with LLMs, we need a suitable dataset of configuration dependencies that is annotated with ground truth labels. We therefore searched for software projects with technologies that have potential configuration dependencies across the entire technology stack and are covered by a previously published dependency-detection framework that allows us to extract these dependencies. We decided to use \emph{CfgNet}~\cite{simon2023cfgnet} as a tool, as it is technology-agnostic and supports many state-of-the-art technologies. For the technology stack, we selected software projects with a microservice technology stack within the Spring Boot ecosystem.

\paragraph{\textbf{Subject Systems}}
The selection of software projects was driven by the usage of the ecosystem and the activity as well as star count in GitHub. This way, we obtain highly practical, real-world software projects for our study. Using GitHub Topics~\footnote{\url{https://github.com/topics}}, we obtain over 60,000 public repositories in the Spring Boot ecosystem. We sorted these projects by stars and included those incorporating at least the following technologies: Spring Boot, Maven, Docker, and Docker Compose. We stopped the selection after identifying 10 suitable projects with these technologies. The resulting subject systems and their characteristics are shown in Table~\ref{tab:subject-systems}.

\input{tables/table-subject-systems}

\paragraph{\textbf{Extracting Dependencies from Subject Systems}}
To get a dataset of configuration dependencies from our subject systems, we apply \emph{CfgNet} to all of them and extract all potential configuration dependencies. For each software project, we randomly select 50 configuration dependencies from the detected ones, resulting in a set of 500 intra- and cross-technology dependencies for our study. The rational for this sampling is that all dependencies must be manually checked in detail to create a trustworthy and correct ground truth. That is, the main author manually reviewed all dependencies and annotated them as either\emph{true}, \emph{false}, or as \emph{borderline} case. \emph{Borderline} cases were discussed by at least two authors until a consensus in favor of a \emph{true} or \emph{false} dependency was found. This way, we created the largest ground truth cross-technology configuration dependency dataset that we are aware of and that have been used in any study. As an important contribution of this work, we make this dataset available for other researchers and tool developers.

==> tables/table-failure-categories-defintion.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[tbh]
\footnotesize
\caption{Eight failure categories derived from a validation failures from vanilla LLMs and RAG.}
\label{tab:failure-categories-definition}
\setlength{\tabcolsep}{3.0pt}
\begin{tabular}{@{}p{1.6cm}p{7cm}p{2.0cm}p{2.cm}@{}}
\toprule
Failure Cat. & Description & Technologies & Actionable\\ \midrule

Inheritance and Overrides & Maven introduces project inheritance, allowing modules to inherit configuration from a parent module, such as dependencies, plugins, properties, and build settings. This means, for instance, while the groupID of a project generally gets inherited and is not a dependency if set explicitly, this is not true if a module is depending on another one. Meaning that in these cases the groupID has to be set explicitly and be the same. & Maven & Provide project-specific information on project structure and module organization \\\midrule

Configuration Consistency & Often values are the same across configuration files to ensure consistency. In this failure category, LLMs confuse equal values for the sake of consistency with dependencies. & Docker-Compose, Maven, Node.js, Spring Boot & Specialize prompt to distinguish consistency and dependency \\\midrule

Resource Sharing & Sometimes resources, such as databases or services can be shared across modules or used exclusively by a single module. Without additional project-specific information on how resources belong to modules, LLMs struggle to identify these dependencies. & Docker-Compose, Spring & Provide project-specific information on available resources \\\midrule

Port Mapping & The ports of an service (e.g., Web server) are typically defined in several configuration files of different technologies, such as \emph{application.yml}, \emph{Dockerfile}, and \emph{Dockerfile}. However, not all port mappings have to be equal (e.g. a container and host port in docker compose). & Docker, Docker-Compose, Spring & Provide examples for port mapping dependencies and non-dependencies\\\midrule

Ambiguous Options Names & Software projects often use ambiguous naming schemes for configuration options and their values. These ambiguities result from generic and commonly used names (e.g., project name) that may not cause configuration errors if not consistent but can easily lead to misinterpretation by LLMs. & Docker-Compose, Maven, Spring & Specialize prompt to create awareness of naming conventions \\\midrule

Context (Availability, Retrieval, and Utilization) & Failures in this category are either because relevant information is missing (e.g. not in the vector database or generally not available to vanilla LLMs), available in the database but not retrieved, or given to the LLM but not utilized to draw the right conclusion. & Docker-Compose, Maven & Add context, improve sources, or improve retrieval and prompting\\\midrule


% Exlusive Dependencies -> Independent Technologies/Services
Independent Technologies and Services & In some cases (e.g. in containerized projects) different components are isolated by design. Thus, in these cases the configuration options between these components are independent, if not explicitly specified.  & Docker, Docker-Compose & Provide examples of dependent and independent cases \\ \midrule

% Inferring Dependencies -> Others
Others & This category contains all cases in which the LLMs fail to classify the dependencies correctly that can not be matched to any other category and share no common structure. & Docker, Docker-Compose, Spring, Maven, Node.js, TSconfig & Provide similar examples if possible \\ \bottomrule

\end{tabular}
\end{table}

==> tables/table-metrics-definitions.tex <==
\begin{wraptable}{r}{6.85cm}
\vspace{-1.0\baselineskip}
\footnotesize
\centering
\caption{Definitions of confusion matrix (CM) terms}
\label{tab:metrics-definitions}
\renewcommand{\tabcolsep}{2pt}
\begin{tabular}{@{}cl@{}}
\toprule
Term & Definition \\ 
\midrule
TP & True config dependency validated as correct \\ 
FP & Incorrect config dependency validated as correct \\ 
TN & Incorrect config dependency validated as incorrect \\ 
FN & Valid config dependency validated as incorrect \\ \bottomrule
\end{tabular}
\vspace{-1.0\baselineskip}
\end{wraptable}

==> tables/table-refinements.tex <==
\begin{table}[]
\footnotesize
\caption{Four potential refinements derived from the analysis of validation failures of vanilla LLMs and the best-performing RAG.}
\label{tab:refinments}
\begin{tabular}{@{}lll@{}}
\toprule
Refinements                                                                                                   & Categories                                              & Technologies                                                               \\ \midrule
Provide project-specific information (e.g., module organization, implementation details, available resources) & Inheritance and Overrides, Resource Sharing             & Maven, Spring Boot                                                         \\
Specialize the prompt  (e.g., distinguish consistency and dependency, create awareness for naming schemes)    & Configuration Consistency, Ambiguous Option Values      & Docker Compose, Maven, Node.js, Spring Boot                                \\
Few-Shot Prompting (e.g., port mappings, dependent and independent cases)                                     & Port Mapping, Independent Technologies/Services, Others & Docker, Docker Compose, Spring Boot, Maven, Node.js, Spring Boot, TSconfig \\
Improve Retrieval and Generation                                                                              & Context (Availability, Retrieval, Utilization)          & Docker, Maven                                                              \\ \bottomrule
\end{tabular}
\end{table}
